A Faster Algorithm for Minimum-Cost Bipartite Matching in Minor-Free Graphs

We give an $\tilde{O}(n^{7/5} \log (nC))$-time algorithm to compute a minimum-cost maximum cardinality matching (optimal matching) in $K_h$-minor free graphs with $h=O(1)$ and integer edge weights having magnitude at most $C$. This improves upon the $\tilde{O}(n^{10/7}\log{C})$ algorithm of Cohen et al. [SODA 2017] and the $O(n^{3/2}\log (nC))$ algorithm of Gabow and Tarjan [SIAM J. Comput. 1989]. For a graph with $m$ edges and $n$ vertices, the well-known Hungarian Algorithm computes a shortest augmenting path in each phase in $O(m)$ time, yielding an optimal matching in $O(mn)$ time. The Hopcroft-Karp [SIAM J. Comput. 1973], and Gabow-Tarjan [SIAM J. Comput. 1989] algorithms compute, in each phase, a maximal set of vertex-disjoint shortest augmenting paths (for appropriately defined costs) in $O(m)$ time. This reduces the number of phases from $n$ to $O(\sqrt{n})$ and the total execution time to $O(m\sqrt{n})$. In order to obtain our speed-up, we relax the conditions on the augmenting paths and iteratively compute, in each phase, a set of carefully selected augmenting paths that are not restricted to be shortest or vertex-disjoint. As a result, our algorithm computes substantially more augmenting paths in each phase, reducing the number of phases from $O(\sqrt{n})$ to $O(n^{2/5})$. By using small vertex separators, the execution of each phase takes $\tilde{O}(m)$ time on average. For planar graphs, we combine our algorithm with efficient shortest path data structures to obtain a minimum-cost perfect matching in $\tilde{O}(n^{6/5} \log{(nC)})$ time. This improves upon the recent $\tilde{O}(n^{4/3}\log{(nC)})$ time algorithm by Asathulla et al. [SODA 2018].

==> dijkstra.tex <==
\section{Fast \dijkstra\ procedure}

%**This section is left over from a previous version, but may prove useful if more elaboration of \dijkstra\ is needed.**\\\\

\newcommand{\induced}{I}
\newcommand{\weight}[1]{d(#1)}
\newcommand{\ind}[1]{I(#1)}

%interval fields
\newcommand{\interval}{\mathcal{I}_\mathcal{M}}
\newcommand{\intstart}[1]{#1_{start}}
\newcommand{\intend}[1]{#1_{end}}
\newcommand{\intmonge}[1]{#1_m}
\newcommand{\intx}[1]{#1_v}
\newcommand{\intmin}[1]{#1_{min}}

This section describes how to compute the minimum cost path in $H'$ from an arbitrary vertex of $B_F$ to an arbitrary vertex of $A_F$ in time $\tilde{O}(V(H'))$, that is, $\tilde{O}(n / \sqrt{r})$.

The graph $H'$ may change completely whenever a dual adjustment is done after \dijkstra\, since this procedure alters the slacks on edges. Therefore, we cannot maintain the edges of $H'$ explicitly. However, we can compute the cost of any edge $(u,v) \in H'$ solely from $H$, $\ty{u}$, $\ty{v}$ in constant time by lemma (sumslacks). This means we can work with $H'$ as if it were explicitly stored, although the implicitly stored edge weights may still change when a dual adjustment occurs.

We are interested in finding the distance $\dist(\cdot)$ to vertices from an arbitrary vertex of $B_F$. The distances will be revealed as we expand a search tree; if the distance to a vertex has not yet been revealed, let it have a distance infinity. All vertices in $B_F$ have a distance 0. For any edge $(u,v)$ in $H'$, we denote the weight of $(u,v)$ as \weight{u,v}. Let an edge $(u,v)$ in $H'$ be a \textit{frontier} edge if the distance to $u$ has been revealed, but the distance to $v$ has not. Dijkstra iteratively selects the frontier edge which minimizes $\dist(u) + \weight{u,v}$. 

Our approach is much like the approach used by \FR in their FR-Dijkstra algorithm. The main differences are that they use multiple layers of dense distance graphs while we use the graph $H'$. However, we show that the graph $H'$ exhibits similar properties to their dense distance graphs. We also propose an implementation of one of their internal data structures that facilitates faster update times. FR-Dijkstra works in $\tilde{O}(V)$ time instead of $\tilde{O}(E)$ time. This speedup arrises from an effective pruning frontier edges. The pruning technique applies to $H'$ as well. We denote $\induced$ as the set of induced edges between two boundary vertices of $H'$. We denote by $\induced_j$ the induced edges between two boundary nodes of $R_j$. By lemma (construct H lemma) the total number of edges in $E(H') \backslash \induced$ is $O(n / \sqrt{r})$. Therefore, we do not need to prune these edges, and the only edges which need to be pruned are those in $\induced$.

For completeness, we describe a high level overview of how FR-Dijkstra prunes edges in $\induced$. 

\subsection{The Monge Property}
FR-Dijkstra makes heavy use of the Monge property. Assume we are given a bipartite sub-graph of $\induced_j$ with two ordered sets of vertices $X$ and $Y$, and all edges are directed from $X$ to $Y$. **Needs a figure**. Such a setup forms a \textit{Monge group}. For any vertex $x \in X$, $y \in Y$ let $\ind{x}$ be the index of $x$ in $X$ and let $\ind{y}$ be the index of $y$ in $Y$. Let $d(u,v)$ represents the length of the shortest path from $u$ to $v$ in $G_S$ using only vertices of $R_j$. The Monge property implies that for any $p,q \in X$ and $r,s \in Y$, where $\ind{p} < \ind{q}$ and $\ind{r} < \ind{s}$, 

\begin{equation}
\label{eq:monge}
d(p,r) + d(q,s) \leq d(p,s) + d(q,r)
\end{equation}

The property applies in our case since the shortest paths from $p$ to $s$ and $q$ to $r$ must cross at some vertex $t$, implying $d(p,r) \leq d(p,t) + d(t,r)$ and $d(q,s) \leq d(q,t) + d(t,s)$. Note that the property still holds upon adding arbitrary weights to vertices, since any such weight would apply to both sides of equation (\ref{eq:monge}). As an implication of equation (\ref{eq:monge}), consider a situation where some $p \in X$ minimizes $d(p,s)$ among all vertices of $X$. Then, $d(p,s) \leq d(q,s)$. By equation (\ref{eq:monge}), this implies $d(p,r) \leq d(q,r)$. This can be described as a "non-crossing" property for shortest paths from $X$ to $Y$.

\subsection{Formation of Monge Groups}

In order to exploit the Monge property, it is desirable to form Monge groups. We use the same strategy as \FR to split the edges of $\induced_j$ into edge dijsoint bipartite subgraphs. For each region $R_j$, we assume we have a circular ordering of the boundary vertices. We will first split the boundary of $R_j$ into two pieces with a roughly equal number of boundary vertices. These two pieces form vertex sets $X_1$ and $Y_1$ of a Monge group. The edge set for this Monge group consists of all $H$ edges in $R_j$ which from some $x \in X_1$ to some $y \in Y_1$. We then recursively split $X_i$ into $X_{i+1}$ and $Y_{i+1}$, and we split $Y_i$ into $X_{i+2}$ and $Y_{i+2}$. Finally, for each Monge group $X,Y$ we will also maintain a mirrored group where $X$ and $Y$ are swapped, containing edges from $Y$ to $X$. Thus, each edge belongs to one Monge group, and each boundary vertex belongs to $O(\log{\sqrt{r}})$ groups in $R_j$. For any Monge group $(X,Y)$, let $X$ be the vertices on the 'left' and let $Y$ be the vertices on the 'right'. **Include a figure**.

In the event that $R_j$ is not connected, we can apply the above procedure on each subpiece. It is possible that $R_j$ has holes, meaning the boundary vertices lie on faces not in $G$. Let $h$ be the number of holes in $R_j$. The $r$-division algorithm guarantees $h = O(1)$. Let the $h$ holes be ${w_1, w_2, ..., w_h}$. In this case, use the above procedure for all edges $(u,v)$ where $u,v \in w_i$. We also create $h(h-1)$ different Monge groups containing all edges $(u,v) \in (w_i \times w_k) \cap E(R_j)$ where $i \neq k$.

\subsection{Operations on Monge Groups}

Within each Monge group $(X,Y)$, we will maintain a set of disjoint intervals $\interval$ indexed on $Y$. For any interval $i \in \interval$, we denote $\intstart{i}$ to be the lowest index in $Y$ contained in $i$. Similarly, we denote $\intend{i}$ as the highest index in $Y$ contained in $i$. Each interval will have an associated Monge group $\intmonge{i}$. Finally, each interval will have an associated vertex in $X$, $\intx{i}$ We will ensure that the set of intervals cover all vertices in $Y$ whose distances have not yet been revealed (assuming some interval in the Monge group has been initialized). Intuitively, each interval $i$ represents the portion of the vertices along the Dijkstra frontier for which $\intx{i}$ may be the best parent among all all vertices in $\intmonge{i}$.

To facilitate the identification of the minimum distance frontier edge, we will maintain a priority queue $Q$. $Q$ will explicitly store all frontier edges in $H' \backslash \induced$. We will also store the intervals from the Monge groups in $Q$ to account for vertices in $\induced$. We will support the following operations within each Monge group $(X,Y)$. The operations are described in detail in \FR's paper. 

\begin{enumerate}
\item 
\textbf{ActivateLeft($x$)}: Add $x$ to the activated set of $X$. The activated set consists of all vertices $v \in X$ for which the total distance to $v$ in the Dijkstra search, $\dist(v)$, has been revealed. A vertex $v$ is added to the activated set when an edge $(.,v)$ is extracted from $Q$ or an interval $i$ such that the result of FindMin($i$)$=v$ is extracted from $Q$.
\item 
\textbf{FindMin($i$)}: Return the vertex $y \in Y$ in the interval $i$ for which $d(x,y)$ is minimized. For any interval $i$, let $\intmin{i}$ be the value returned by this function. This function is supported by a range search structure described in section \ref{rangesearch}. This is used as the value of an interval entry in $Q$.
\item 
\textbf{ExtractMin($x$, $i$)}: Let $y$ be the result of FindMin($x$, $i$). If $y$ has not been visited, set $\dist(y)=\dist(x) + d(x,y)$ and activate $y$ in all other Monge groups for which $y$ is on the 'left'. Add any frontier edges of $H \backslash \induced$ to $Q$. Mark $y$ as visited. Split the interval $i$ into 2 intervals such that all vertices in $i$ are included except $y$.
\end{enumerate}

\subsection{Interval Minimum Search}
\label{rangesearch}
In each Monge group $(X,Y)$, \FR assume the presence of a range tree structure for every $x \in X$ that for any interval in $Y$ returns the $y \in Y$ in the interval which minimizes $\weight{x,y}$. They construct this structure independently for each $x$. Computing this structure for all vertices in $X$ would require time proportional to the number of edges in the Monge group. After the Dijkstra procedure, the dual values for many $\ty{\cdot}$ may change, and many of these range tree structures would have to be reconstructed. This could take $\tilde{O}(n)$ time, which is insufficient. To remedy this, we propose an alternative structure that accomplishes the same purpose, but can be built in time $\tilde{O}(n/\sqrt{r})$. This means all range search structures could be rebuilt in time $\tilde{O}(n/\sqrt{r})$ prior to a \dijkstra\ search without increasing the complexity of the \dijkstra\ search. The speedup comes from exploiting the Monge property in order to compute the solutions for many vertices in $X$ simultaneously as opposed to independently. We assume that we have access to $H'$ for the creation of this structure. We will explicitly compute the solution for a fixed set of $O(|Y|)$ intervals and use $\log{|Y|}$ such intervals to answer an arbitrary interval query. 

First, we build a balanced binary tree $T$ of the indices of $Y$. In this way, the leaf node each represent an interval consisting of a single node, and each internal node corresponds to an interval spanning from the leftmost node in its subtree to the rightmost node in its subtree. We will compute the solution for each tree node's interval for all values of $\intx{i}$. To perform an arbitrary query for an interval $i$, we find the least common ancestor of the leaf nodes corresponding to $\intstart{i}$ and $\intend in T$. Let this be $r$. Let $P_{\intstart{i}}$ be the path up $T$ from $\intstart{i}$ to $r$.  Define $P_{\intend{i}}$ similarly. Then there exists some subset $S$ of the vertices in $P_{\intstart{i}} \cup P_{\intend{i}}$ such that.
\begin{enumerate}
\item For any $s \in S$, the interval corresponding to $s$ is contained in $i$.
\item All intervals of nodes in $S$ are disjoint.
\item The intervals of nodes in $S$ together span $i$.
\item $|S|=O(\log{|Y|})$
\end{enumerate}

$S$ can be found simply by taking all vertices in $P_{\intstart{i}} \cup P_{\intend{i}}$ for which condition (1) holds. Therefore, the query for an arbitrary interval $i$ can be answered by taking the minimum over interval queries for all nodes of $S$.

We now describe how to compute the solution for each node $t$ in $T$. For each node, perform a divide and conquer algorithm using the Monge property as follows. We will use the entire set $X$, but only the subset of $Y$ that is in $t$. Let this subset be $Y'$. The Monge search will take $O(|Y'|\log{|X|})$. Find the middle vertex of $X$, $x_{mid}$. Linearly search through $Y'$ for the vertex $y$ which minimizes 
$\weight{x_{mid}, y)}$. Then recurse on the top half and the bottom half of $X$. We  can conclude from the Monge property that the top half of $X$ need not consider any vertex below $y$. Similarly, the bottom half need not consider vertices above $y$. 

The time spent for any subproblem $X^*,Y^*$ is $O(|Y^*|)$. The total time spent for any layer of the recursion is $O(|Y'|) + O(X_r)$ where $X_r$ is the number of subproblems in the recursion layer. This could be problematic if $X_r \geq |Y'|$. However, if this is true, then there must be some subproblems $X^*, Y^*$ with only a single vertex $y$ in $Y*$ remaining. When this occurs for a subproblem, we simply store the interval representing $X^*$ and associate it with $y$; the problem need not be subdivided further. 
The number of such subproblems where this can occur is $O(|Y'|\log|X'|)$. To see this, consider the fact that the recursion tree forms a balanced binary tree on the indices of $X'$. \mnote{More proof is needed here}
